Structure-Guided Image Completion with Image-level and Object-level Semantic Discriminators

Structure-guided image completion aims to inpaint a local region of an image according to an input guidance map from users. While such a task enables many practical applications for interactive editing, existing methods often struggle to hallucinate realistic object instances in complex natural scenes. Such a limitation is partially due to the lack of semantic-level constraints inside the hole region as well as the lack of a mechanism to enforce realistic object generation. In this work, we propose a learning paradigm that consists of semantic discriminators and object-level discriminators for improving the generation of complex semantics and objects. Specifically, the semantic discriminators leverage pretrained visual features to improve the realism of the generated visual concepts. Moreover, the object-level discriminators take aligned instances as inputs to enforce the realism of individual objects. Our proposed scheme significantly improves the generation quality and achieves state-of-the-art results on various tasks, including segmentation-guided completion, edge-guided manipulation and panoptically-guided manipulation on Places2 datasets. Furthermore, our trained model is flexible and can support multiple editing use cases, such as object insertion, replacement, removal and standard inpainting. In particular, our trained model combined with a novel automatic image completion pipeline achieves state-of-the-art results on the standard inpainting task.

==> sections_tpami/related_short.tex <==
% \vspace{-0mm}
\section{Related work}
% \vspace{-2mm}
\subsection{Image Inpainting and Guided Image Inpainting}
% \vspace{-2mm}
%Image inpainting has a long-standing history.
Early image inpainting methods leverage patch-based copy-pasting~\cite{Image_quilting,kwatra2005texture,patchmatch,cho2008patch,image_melding} or color propagation~\cite{ballester2001filling,chan2001nontexture,shen2002mathematical,criminisi2004region} to fill in the target hole. Those methods can produce high-quality textures while completing simple shapes but cannot hallucinate new semantic structures.
% due to the lack of mechanism for modeling the high-level semantic information.
%With the development of deep generative models
Recently, deep generative models have shown promising results on image inpainting.
%By training generative models~\cite{gan,esser2021taming} on large scale datasets, the learned models can capture higher-level representation of images and facilitate visually plausible predictions.
Inspired by ~\cite{pathak2016context} that trains an encoder-decoder network to completes the missing region of an image, numerous approaches have been proposed to improve the learning-based hole filling. The proposed mechanisms including multi-stage networks~\cite{deepfill,MEDFE,hifill,ict,profill,edgeconnect,foreground_aware,yang2020learning,song2018spg}, attention mechanism~\cite{deepfill}, dilated convolution~\cite{iizuka2017globally,deepfill}, Fourier convolution~\cite{chi2020fast,lama} expands the receptive field of the generative models, allowing better contextual feature propagating while enabling better inpainting quality.
Recently, modulation-based methods~\cite{comodgan,cmgan} further improve the global context modeling for image inpainting.
In addition, probabilistic diffusion models~\cite{ho2020denoising,saharia2021palette,lugmayr2022repaint} and vision transformers~\cite{ict,zheng2021pluralistic,zheng2021tfill} have also shown promising results on image inpainting.
% \vspace{-4mm}
% \subsection{Guided Image Inpainting}
% \vspace{-2mm}
%Completing the complex semantic structure of natural images is inherently challenging.
%Despite showing impressive results on completing background or partial objects, image inpainting methods would often lead to obvious structural artifacts for large holes, 
%Different from image inpainting, g
Guided inpainting leverages additional structural guidance to improve image completion of complex semantic structures while providing tools for users to manipulate the inpainting outcome. 
In the literature, edge~\cite{deepfillv2,edgeconnect,foreground_aware}, color~\cite{faceshop,face_editing2019} or gradient maps~\cite{yang2020learning} are used to guide the image completion process.
To provide semantic-level control for inpainting, semantic segmentation~\cite{song2018spg,hong2018learning,sesame} is also used as a guidance map for more controlled inpainting. In addition, exemplar patches~\cite{zhang2022inpainting} are also used as guidance for inpainting.
%Specifically, Song \etal~\cite{song2018spg} predict semantic layout to improve the realism of the generated layout. Hong \etal~\cite{hong2018learning} leverage semantic segmentation to manipulate the generated contents, Ntavelis \etal~\cite{sesame} leverage a local semantic layout to control the inpainting outcome for scene manipulation.

% \vspace{-4mm}
\subsection{Discriminators for GANs}
% \vspace{-2mm}
The initial Generative Adversarial Networks (GANs)~\cite{gan} leverages a multilayer perceptron (MLP) to predict the realism of the generated images. 
Since then, there have been rapid advance to achieve photo-realistic image synthesis.
Specifically, patch discriminator~\cite{isola2017image,li2016precomputed,deepfillv2} is proposed to predict the realism of the generated patches in local regions.
Later, the StyleGAN-based discriminators~\cite{stylegan,stylegan2} leverages strided convolution combined with a fully connected layer to generate realistic images. 
Motivated by contrasitive learning~\cite{chen2020simple}, several works~\cite{kang2020contragan,zhang2021cross,jeong2021training,yu2021dual} design discriminators to predict the pairwise relations between different modalities or the real and fake samples. 
Likewise, the patch co-occurrence discriminator~\cite{park2020swapping} predicts the similarity between the output patches and the reference style image.
To enhance the recognition capacity of a discriminator, recent works~\cite{sauer2021projected,ensembling-gan} leverage pretrained visual features to enhance the semantic understanding of a discriminator for unconditional generation.

